Coherent3D: Coherent 3D Portrait Video Reconstruction via Triplane Fusion

Recent breakthroughs in single-image 3D portrait reconstruction have enabled telepresence systems to stream 3D portrait videos from a single camera in real-time, democratizing telepresence. However, per-frame 3D reconstruction exhibits temporal inconsistency and forgets the user's appearance. On the other hand, self-reenactment methods can render coherent 3D portraits by driving a 3D avatar built from a single reference image, but fail to faithfully preserve the user's per-frame appearance (e.g., instantaneous facial expression and lighting). As a result, none of these two frameworks is an ideal solution for democratized 3D telepresence. In this work, we address this dilemma and propose a novel solution that maintains both coherent identity and dynamic per-frame appearance to enable the best possible realism. To this end, we propose a new fusion-based method that takes the best of both worlds by fusing a canonical 3D prior from a reference view with dynamic appearance from per-frame input views, producing temporally stable 3D videos with faithful reconstruction of the user's per-frame appearance. Trained only using synthetic data produced by an expression-conditioned 3D GAN, our encoder-based method achieves both state-of-the-art 3D reconstruction and temporal consistency on in-studio and in-the-wild datasets. https://research.nvidia.com/labs/amri/projects/coherent3d

==> definitions.tex <==
\newcommand{\model}{$\pi$-GAN\xspace}
\newcommand{\siren}{{\sc siren}}

\newcommand{\pose}{\xi}
\newcommand{\coord}{\mathbf{x}}
\newcommand{\noise}{\mathbf{z}}
%\newcommand{\dir}{\boldsymbol{\nu}}
\newcommand{\dir}{\mathbf{d}}
\newcommand{\density}{\sigma}
\newcommand{\col}{\mathbf{c}}

\newcommand{\generatorparams}{\theta_G}
\newcommand{\generator}{G_{\generatorparams}}
\newcommand{\discriminatorparams}{\theta_D}
\newcommand{\discriminator}{D_{\discriminatorparams}}

\newcommand{\filmmult}{\boldsymbol{\gamma}}
\newcommand{\filmadd}{\boldsymbol{\beta}}

% representation
\newcommand{\implicitlayer}{\phi}
\newcommand{\implicit}{\Phi}
\newcommand{\implicitparams}{\theta}
\newcommand{\nonlinearlayer}{\sin}
\newcommand*\rot{\rotatebox{90}}


%\newcommand{\siren}{SIREN}

% \newcommand{\reducespace}{\vspace{-3pt}}

\newif\ifdrafting
\draftingtrue % Show comments
%\draftingfalse % Remove comments

\ifdrafting
    \newcommand{\mw}[1]{\textcolor{magenta}{[Mike: #1]}}
    \newcommand{\mc}[1]{\textcolor{magenta}{[Matthew: #1]}}
    \newcommand{\sd}[1]{\textcolor{blue}{[Shalini: #1]}}
    \newcommand{\js}[1]{\textcolor{green}{[Josef: #1]}}
    \newcommand{\kn}[1]{\textcolor{red}{[Koki: #1]}}
    \newcommand{\xt}[1]{\textcolor{orange}{[Xueting: #1]}}
    \newcommand{\ms}[1]{\textcolor{green}{[Michael: #1]}}
\else
    % Remove comments
    \newcommand{\mc}[1]{}
    \newcommand{\sd}[1]{}
    \newcommand{\js}[1]{}
    \newcommand{\kn}[1]{}
    \newcommand{\xt}[1]{}
\fi

% \newcommand{\myparagraph}[1]{\vspace{-8pt}\paragraph{#1}}

